Latency optimal storage and scheduling of replicated fragments for memory-constrained servers

We consider the setting of distributed storage system where a single file is subdivided into smaller fragments of same size which are then replicated with a common replication factor across servers of identical cache size. An incoming file download request is sent to all the servers, and the download is completed whenever request gathers all the fragments. At each server, we are interested in determining the set of fragments to be stored, and the sequence in which fragments should be accessed, such that the mean file download time for a request is minimized. We model the fragment download time as an exponential random variable independent and identically distributed for all fragments across all servers, and show that the mean file download time can be lower bounded in terms of the expected number of useful servers summed over all distinct fragment downloads. We present deterministic storage schemes that attempt to maximize the number of useful servers. We show that finding the optimal sequence of accessing the fragments is a Markov decision problem, whose complexity grows exponentially with the number of fragments. We propose heuristic algorithms that determine the sequence of access to the fragments which are empirically shown to perform well.

==> sections/ComputationOfMeanDownloadTimes.tex <==
\newpage
\section{Computation of mean download times}
\subsection{Simple Codes}

Given $(n,k,s)$ code, where $s$ is the number of servers, $k$ is the total number of fragments, $s=k$ and $s\alpha$ is the maximum number of symbols that can be stored per server, what is the best way one can place these $n$ coded symbols across the $s$ servers?

This is considered for an example where $s$ = 4, $k$ = 4 and $\alpha$ = 1/2.

Considering a scenario where a file $F$ is broken into fragments: $F_1$, $F_2$, $F_3$ and $F_4$ and stored in any of the below configurations:

\begin{center}
Server 1:\quad$F_1$\quad $F_2$\quad\quad\quad Server 1:\quad$F_1$\quad $F_4$\\Server 2:\quad$F_2$\quad$F_3$\quad\quad\quad Server 2:\quad$F_2$\quad$F_1$\\Server 3:\quad$F_3$\quad$F_4$\quad\quad\quad Server 3:\quad$F_3$\quad$F_2$\\Server 4:\quad$F_4$\quad$F_1$\quad\quad\quad Server 4:\quad$F_4$\quad$F_3$\\
\end{center}   

There are many ways of getting the whole file from the servers leading to different number of useful servers after a particular number of fragments are received. Specifically: 

\begin{center}
\begin{tabular}{|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{2cm}|}
\hline
\multicolumn{4}{|m{2.8cm}|}{Number of pieces received vs number of useful servers} & Number of symbol combinations (out of 104) & Probability of symbol combinations\\
\hline
0 & 1 & 2 & 3 & $N_s$ & $P_s$\\
\hline
4 & 4 & 4 & 2 & 32 & 1/128\\
4 & 4 & 3 & 2 & 72 & 1/96\\
\hline
\end{tabular}
\end{center}

While another two configurations:

\begin{center}
Server 1:\quad$F_1$\quad $F_3$\quad\quad\quad Server 1:\quad$F_1$\quad $F_4$\\Server 2:\quad$F_2$\quad$F_4$\quad\quad\quad Server 2:\quad$F_2$\quad$F_3$\\Server 3:\quad$F_3$\quad$F_1$\quad\quad\quad Server 3:\quad$F_3$\quad$F_2$\\Server 4:\quad$F_4$\quad$F_2$\quad\quad\quad Server 4:\quad$F_4$\quad$F_1$\\
\end{center}

give the following result:

\begin{center}
\begin{tabular}{|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{0.7cm}|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{2cm}| }
\hline
\multicolumn{4}{|>{\centering\arraybackslash}m{2.8cm}|}{ \centering Number of pieces received vs number of useful servers} & Number of symbol combinations (out of 96) &  Probability of symbol combinations\\
\hline
0 & 1 & 2 & 3 & $N_s$ & $P_s$\\
\hline
4 & 4 & 4 & 2 & 64 & 1/128\\
4 & 4 & 2 & 2 & 32 & 1/64\\
\hline
\end{tabular}
\end{center}

The mean time of service for these two configurations over all possible sets of remaining useful servers is:$$T= \sum_{s} N_s P_s \mathbb{E}T_s$$
where:-

\begin{flushleft}
$N_s$ = Number of symbol sequences with same set of remaining useful servers.\\
$P_s$ = Probability of the symbol sequence.\\
$\mathbb{E}T_s$ = mean time to download sequence
\end{flushleft}

For the first table, the mean time of mean time of service = 21/16 = 1.3125\\
While for the second table, the mean time of service = 11/8 = 1.375\\~\\ 
Which means that for the latter set of configurations, on average, it takes more time to serve the whole file as compared to the former set of arrangements. 

Thus, for this particular example:-

\begin{center}
Server 1:\quad$F_1$\quad $F_2$\quad\quad\quad Server 1:\quad$F_1$\quad $F_4$\\Server 2:\quad$F_2$\quad$F_3$\quad\quad\quad Server 2:\quad$F_2$\quad$F_1$\\Server 3:\quad$F_3$\quad$F_4$\quad\quad\quad Server 3:\quad$F_3$\quad$F_2$\\Server 4:\quad$F_4$\quad$F_1$\quad\quad\quad Server 4:\quad$F_4$\quad$F_3$\\
\end{center}

Will be optimal ways of storing symbols across storage constrained servers for implementing repetition coding.

